AEGR: A simple approach to gradient reversal in autoencoders for network anomaly detection

Anomaly detection is referred to as a process in which the aim is to detect data points that follow a different pattern from the majority of data points. Anomaly detection methods suffer from several well-known challenges that hinder their performance such as high dimensionality. Autoencoders are unsupervised neural networks that have been used for the purpose of reducing dimensionality and also detecting network anomalies in large datasets. The performance of autoencoders debilitates when the training set contains noise and anomalies. In this paper, a new gradient-reversal method is proposed to overcome the influence of anomalies on the training phase for the purpose of detecting network anomalies. The method is different from other approaches as it does not require an anomaly-free training set and is based on reconstruction error. Once latent variables are extracted from the network, Local Outlier Factor is used to separate normal data points from anomalies. A simple pruning approach and data augmentation is also added to further improve performance. The experimental results show that the proposed model can outperform other well-know approaches.

==> AEGR Article/.git/objects/11/f3e72cce97c04d82079ad49f9afaefb20085b1 <==
x•ŽA
à E»ö³/5ŽF(¥]÷£Ž­4‰!1=Ó#"¿øðø~¬ÓTè^ÚÊ!$#³V™{£Ùy(JŸX2å'Ãt,´Žb¡•çì%fÄl£1}f;"8脉¢Jžú!;MííUWxж\Þ¿
G¸Üž•±‹uº'B‡Vi,œå ¥8èq¯ñߢ¸§Ÿ²í4–Z©3,cm['¾'K5

==> AEGR Article/.git/objects/3a/d8f87e37b9baacd239cf9b336fc29e28eff4e9 <==
xmR]OÃ õuþ
ž|[2hK[ßÔE³h"uú ÆPËV'
Üé´á¿ý0Î΅{.çÀ¥lt‰'Ÿ°Rl¥j—pOõó鄽òH­Ú¢¨Àec'Þ Š·¬ó"†—¢é‹ÎÇý—ëó¶Ñ"aå—ë•}ÃÍÁµ¬'J|È
j×6¨¡nÂêѼ—CgèZpØa}ÈÞAïZV—úÐ2f¨0\*©¶î÷në:çþ/ŽÈ¨##Ǝ
,î‹/‰	&³€Ñ,K=F$%w¡@%à¢
Þp'd%'šÐµ^®§ËKœNŽŠâ8Î=fGé†[oCYm7†¢ÊÈ
"
ŸG'f£øru7½Ï;
ñsS"qDé(½Úñ·Ò7-¤ƒw'Ó ŸÆx½*Ö8šÎ'DÜ]2I;‡i–{‡^"	U…ž÷-<—þß|·¡®7

==> AEGR Article/.git/objects/52/eb229506f8d14753ded4be334a28724c2780bd <==
x•TMo7íY¿'=ØP.–Ÿ»›Sª-Š&'aÙÉ!
j—–ˆR¤Êå"¶·úïáª]9E'H€|óæ͛Yn\Ø*ýæ'Ü8£;Ctے´3ä!8>[¿%ÑüÑÛhZrÐÍïzk:'y
}$mhú½ñ‰¢Ñû3¯fdÝwæ"¶Qv¶y<ÎÖ³µ~HPÇgëF'
~X˜¤­ëHxÈi+Òê:RG€§%Öçcóx0Ñb®¸œÞ7r½Bø'ÄjG&¸¦³Ïf‡u\¿÷Ÿm›vÇáÛãpq¦¤w:÷g3þŽ³pà"^ï
¹$"èýÐ|~Ž
üËð=J^¯ÉƒÑ©‡Œkã[Ԕ¡ÿ|µõh-"Cº¯ˆ|§…ŠÁ¸¯½3]ú¯¤ d½sٍ֛ñ»µàÿ%¡
&JØ8e°–¬"ijծOÉ¡E5^1…ˆŠâJ…,
Ä\Ǹ{J»½ÕpÊ$™¤ˆã¸(Ĝr®0=8|—D"+3¼¦T3ŽÐ_}2ћtÝfeRVpG°‰yE)¸\½¹úm±˜ßÄ°1ß!ˆ¡rÅ3•U'Ï(gçèEXMغPbLeJªêsì-{3aÍõP)F³d]cïÙ턕'eÕ<‹¯Ë2C÷WË×TÎMìr@t²æXn¥ °C‰Sĵ×g!B‰\ Í%@µc7¦×ð·!Ä)‹P£5TJÌY–Pʋ,›3j™™òlŽª˜úBÓO`€¦%͍§e…åW5¯sK'M¿Ÿws¡Æ6Õ‹©Õ¿ª¸5Mð^Û®Ó¾Û<ª;µ™sTJÔôe-«q®	íYŒåh™Àɔ%å_È{â~Ò&dãðxB*°ëÇ»{ʯ(Ÿ¿³±Oύœ¢«Tðq`ápóÛMÈØ|[rŽƒÌD›œ°E=_'GÙU(ʪ™ƒ‰ƒ¹ÒQFQÍßöхdTµªrC2Nßߋèb/èé-ƒ·ú/¹y¶ 

==> AEGR Article/.git/objects/61/55879fdd82340940e53d3165f7c2e3f5208cda <==
x•'ÝnÂ0…wOáI\©RcÚTžbwMi #Kª4?ï¾$-]…Ʀ]Uv¿c;öɄÊ`>ïҌm¸¬×|Siv^ÞoWÃA›£L¦ÏÃÁ%aøîTpj<)¸d@I'hUÉ<ôá»â²‰ÑœÈ`ð0IŒ0ýÍ×ö¤Tð"ˆ¦a"Ñã4£¦Áƒih/É5ÙÃҗÞóÜlŒž
³' š £1P®©í`4ûCÿ+ø½C´h^܌£fªÍüXQdG´3¹ ÷E-NÓ꽤¹KI5/LÉOÌßÁ-dI•P:É¡;¿ŠAªœA=:ŒÎ]¿+÷°ÓmlÒÎ
v¹ÄUÁ(FF"®yu»ª½›[Æ7ûÙ²LæõÕ]ªï4ëG—êܘZÓ®dýºeP]yC'ZŒ"œ©Œb'Ú•8÷¦'dL8‡?ûßoÄîҗlMÿ:~ñæ

==> AEGR Article/.git/objects/75/dafc04d57b11ccae875f79916681b92d0aff76 <==
x"Qo›0Ç÷
Ÿâö–vASÒt"ДîeÚ¦V{jªé0.X5vdœ.ñÝg¢5y
èîw¿;›£ª€Uš}جâ²æÕN³Ëá±þø"ʤašËʚ¸5\Éþ‡Ò
Þ²ð•i¬´TiêÒØ+Šº\h˜ÑœáF`Á"ƒžjþøÛþò¶åÔØÞCL"îy;<†AÐùr'íʱ_`Ÿ®@=™Ö'¿¼45I"­™Ä½áô…"hð EœÐfòÚ®)"àö@•ÒeKúü÷×~iFykÏÁ]ANéN#톩L°ŠI;ˆé#=Òϒ8‹æIœf‡$"´VšH¥MMT‰]#[2O]VðÚ×Ër+"'à
k¡·`æg±ÐåòfïfJ⥗Ül©
æsž-¾œƒ=AZ×á'#\r>.NV‹Å	3¾ñ'çÆËÅÍ1;ÎV·góÝ1ß݀sGìíõÕ	v•]ýǎßÿyÁÃü!_ræhݯ!Ê×ßînñìGíýڅÞ<ZK¯þ¶Ë÷.

==> AEGR Article/.git/objects/85/0c843b0ec99fd4ca316376c74b7519f218d0c5 <==
xÍTMkÜ0íyÅ\
I Ûf驐ÃB7Ké%lC/uYÆòØÐJFgSŒÿ{G²irؤ"äЛ%ϼžJëK¸\}\½)JjØ
57} ‹q1¯c_N[ã°\}("îåȕ´ã 0ä"»Fo±}EPsˆ|À†RѼÝìZ6ñGn¿º\®
ˎòêçpiãûëÞÚý—"êHÖUܯ7ûۀì"äɐy±önXo²‹%Ù¤ü"ª}—éU?¹jxP¿(ښí\E2ÞU¯gk»{ÖØvwÂÚ¤áõ½½db7¡wTýËÌàlê9?áðÞI‡ßs.Ÿœ£™/öwŽ=ZŽ˜®9tÖø¤%°(:¸ÃÀXZŠp–v§ÊÑCM(àxšÔ€F¨'ò D>t–`½ÔkŒ6zýÞî@ñåm	·
纆 óì$B N+:PYÊzlYÁuiû•éóA«g"	ØôáN»Qr«ø.‹	Ü´¢õíP—"¦UCéÒ'¥b£Žc®ÿúyÂR3ðúéLöÎdȄq1þcØÈ~

==> AEGR Article/.git/objects/88/aa20629c23c630ce9b601a3646fb2d760d5fad <==
x•ŽKn!D³æ½dñ™h)²¼Ï)€nlD¾¿É¢Z"êIUªÜ£N°[ø˜Cˆ2ú@ì7''6ç¬-iJû–ón'uR¿qH›v,äµxL'I\ñÚlèÐOìž'‡U|ÍGðÏáëçÏҒÔÛýˆõyÉý¸'AO½ÕŸ:h­]÷¦ü»¨"3äÞʳæ	½@mkEÎyBlCÊJ-ËyQo]lO 

==> AEGR Article/.git/objects/8a/1605731e1c637f9c448cd4c9ede2eebbf9d201 <==
x]SÛnÛ0Ý3¿'ÀtÝǎÇÖíZìeÀöÐݞ
Ù¦c¡²äIr"ôëGËiwq[:âåð*•)1‰‹å‹ÛV:äÿ•,oéÇ¿'uÒhŒ£¢¨ñ5cøI>.ã$?‡¢•ôÇ-vâp缕zç.'x|fØ
×Þ9ùHÿ"½•]äë8.à¶%ô¦Ÿ+z …b8H%…=b#mqñÕqúŽpV"ü#¹øhÌN^[&±øÒ^/.oðÒzY)ZDž½¨}×/>^I²X"§ÊŽ¹áåà͍®LÍqQèwVԒ´GËB©³¼œ?r¦‰‰$"o£Òy¸ž©¸é_&[Œ¢…¥†,éŠ\Tʾ«9Ý|^	}æ97ai|‹F
…ÄzèJ&ØHR5+®ñÊÒ å~šáŒfŸ—kdnV'›þõ$ù&ý|¼«©'šêy3è©Le*1ÖûŸC–fxjû1"|"¯°j…•çºg0Šá¹å •¿c>O!¹¥°2ƒön†yš&#[Æf(,máçs†—ð~\¤Éލ‹ގŸ$YÁ<Xðfü®ó
lƒO',Suõd¥©_§Ë
Œé"ìiÖÀ,õŽ¢Š5ÿÙțHjxO‡ÔC¯$«0«4êz–\54ÆvÂGZt"E^€l¦ÈñztŒ]µöû°|"Ñ:éÆiš¶+дW܅°ÍcàΆàîɼ7}Xô–DWªÉ6~°²™˜Åðk0'Î1¸{9ù¤Ë58/ªûžÁñš…}–eàöb2MŠ5ð
ð'"½óíÉ! œ¶'‡'äD'†g•cØOLØ·|ÿš»µ—õ)wgoŸ•f­^óýµ"{á0áwúsø
èŽGI

==> AEGR Article/.git/objects/97/bcb8bdf8b472a442aa9c2ca07aba86b100c72e <==
x+)JMU02°`040031QÐs	Ž.É/Jeت4ïNbuÆ¿®ÿ_ˎ|3aÆ Pp
ufx¶èt TÔ3™YÖªF‡OµiОø"ìåÌ°Ï?bµåiI¦¤Æwm}+íŽÉŸ¾È'
qcȳeÏ\Î&§ñåÌÄK©œ'ïaö¥&¦ä¦ê¦ê¤¤1lYù{Ç¥ۂÿ)h<âª4êsêN¨º,°º»Ê—~¿«ýQ0óºsãµ}îגŒrìVv

==> AEGR Article/.git/objects/ae/6073afc8083b8bddf952c5c5adb479536b0c15 <==
xíWMO1}Ucäè±@7$Æx\Èbď«,n"BX0r۟b½hÐÌ$Ó7~¼Ð-M‡ãԞÖNÎ@1ù}
¨Ò,SK6ŸˆÄE×d'xJDãÆHà3dx]ËV‡2 lrv+蠋6Z<½Ëó;™¥íy>›2ÞbtÜë"Ü`Œ!æñœçì'è1Ö£uÍ~†©ó>ѓÓî!
šaÀœsVñÀ2XÖNé}¡áìG¨£É¬KFëŒÎï»ìWn$©"y7¯¼V¾ÏÉÞn9VŸ³N¸ïÓ#<‡µq¦3²÷Œ?ÁÀ×{øÛö»Ôõü<¼³EÊ{µU"e`ɀ|,U0XxtŸ6î	@"¿NhË[BjlÀ8`á'Šñ¥D_jÂÃørúmȋ}9Lx|˜0³	/ãfçøÖ¥ÃĵU"Uv}·*÷sóûµH{ʀ2ð¯0¥¤›4¸¥p·®mNîZK½£ŠH^áѕ°	×±3ä*>¤:åAŒé¡èGƒ6ÊÀ¯2ðƒ"n~

==> AEGR Article/.git/objects/e3/3b7593655a7e982aa8fe5b849f60bd2abdda0d <==
x]SÉnÛ0íy¾b€HÓÚZ¬Ä–Œ¦@Òí!E{H·"AI#‹Eª$ÙùúŽ–¤‹lHä㛙Ç7d®LŽq"®ŸÝÖÒ!ÿ¯d~K?ø¬"FcdY‰/ÃyO¸ŠâôމVҷ؈ÃÎy+õÞ]ÄÑð,°®Þ9ù@ÿ"­•
]¤çQ"ÁmMèM»TtO
EwJ
{ÄJ*ÚbøÕqùðN8+rþ'?³W"×–E"_êëðò=^Z/EaàéЊÒ7mx‰¹•%~dñš<~ØÉ'òµ)±2o"Ýs.á…#ï.?
rþÈ%&	'ˆ¼
rçaàåÌWðy¼Å -UdIä'\æð]XÍ,—…Ð';fçÆ×xoT×
]¢îšœU'TÉVk¼²Ôi¹‡Ÿ¦;ag9¦ÄUŠ¤ÙNrÀ¿ž8ݬ±—»'*©©\Vž¶¥L!†ýý°>_áÜŽc%Ù*9âVžÍ]À ÉsòN*¿c=)yJaa:íÝÓ,KµŒ-PXÚÂ.—˜E	¼I'À›aÁëá¯bXŽŒ^
ßuÃvŒá¥DY-YiÊÃjÁP.ðǖF`•«Ô{

öüdo©ýˆpôóbe×*É.LÀÙ&jZ™éyÜòFø@‹fbd	Èj'ŠSà¤Csî`û&R
tŽÛ;M7 ©W܅qšfÀ"»GzkÚq³I­%Ñäj"ÇÐvVV"´~uf»"SPr¶çEq7¦à…ŽápÁÆù†/ëÅD]E)ðÙ÷"½÷õ0"\¶'‡GdÖÁ"Íôӑ)1ô5ß¼qœ­¡—圍ÛÓÛ'«Ó^ò͵"½pó{<õ§ðæxC•

==> AEGR Article/Figures/AEGR_pseudocode.tex <==
\begin{algorithm}[t]

\SetAlgoLined
 
 \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
 \Input{$D$: a dataset with $n\times m$ dimension \\
 $e \leftarrow$ number of epochs}
 \Output{$D'$: a dataset with $n\times m'$ dimension} 
 \BlankLine
 
 initialise: $k \leftarrow$ GR start point\;
 $LGS =$ list of gradient scores\;
 \For{each epoch}{
	 \For{each point/mini-batch in $epoch_j$}{
		 \If{$j > k$}{
		 	\For{each layer}{
			 	\If{bottleneck}{
			 		$GS_j \leftarrow ||n||_F$\\
			 		$LGS \leftarrow GS_j$
			 	}
			}
		}
	 }
	 $Max_{GS} \leftarrow$ Max $GS$ in $LGS$ ;\\
	Bacpropagate inverted $Max_{GS}$;\\
	Shuffle the batches;
 }
 $D' \leftarrow$ the bottleneck of the last epoch
\caption{AEGR}
\label{alg:AEGD}
\end{algorithm}


==> AEGR Article/Figures/AE_Layout.tex <==
\begin{figure}[!h]
\begin{center}
	
	\begin{tikzpicture}[scale=0.8,line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
	\clip(-4.83199028842192,-3.350560119718393) rectangle (5.188918188289323,2.667106384609909);
	\draw [line width=1.2pt] (-4.,-2.) circle (0.32802438933713446cm);
	\draw [line width=1.2pt] (-4.,2.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (-4.,1.) circle (0.32802438933713435cm);
	\draw [line width=1.2pt] (-4.,0.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (-4.,-1.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (-2.,1.) circle (0.3280243893371345cm);
	\draw [line width=1.2pt] (-2.,0.) circle (0.3124099870362662cm);
	\draw [line width=1.2pt] (-2.,-1.) circle (0.31240998703626616cm);
	\draw [line width=1.2pt] (0.,0.) circle (0.3124099870362662cm);
	\draw [line width=1.2pt] (2.,1.) circle (0.32802438933713435cm);
	\draw [line width=1.2pt] (2.,0.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (2.,-1.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (4.,-2.) circle (0.32802438933713446cm);
	\draw [line width=1.2pt] (4.,2.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (4.,1.) circle (0.32802438933713435cm);
	\draw [line width=1.2pt] (4.,0.) circle (0.3124099870362663cm);
	\draw [line width=1.2pt] (4.,-1.) circle (0.3124099870362663cm);
	\draw [->,line width=0.8pt] (-3.671975610662866,1.) -- (-2.3272978670955706,0.9781801421936286);
	\draw [->,line width=0.8pt] (-3.6875900129637342,0.) -- (-2.312409987036266,0.);
	\draw [->,line width=0.8pt] (-3.687590012963734,-1.) -- (-2.311616059483331,-1.022258289963095);
	\draw [->,line width=0.8pt] (-1.6875900129637338,0.) -- (-0.3124099870362662,0.);
	\draw [->,line width=0.8pt] (0.3124099870362662,0.) -- (1.6727021329044296,0.9781801421936286);
	\draw [->,line width=0.8pt] (0.3124099870362662,0.) -- (1.6875900129637338,0.);
	\draw [->,line width=0.8pt] (0.3124099870362662,0.) -- (1.6903305043977526,-1.0412892660802997);
	\draw [->,line width=0.8pt] (2.3257776205028176,0.9616732211173156) -- (3.67270213290443,0.9781801421936286);
	\draw [->,line width=0.8pt] (2.312409987036266,0.) -- (3.6875900129637342,0.);
	\draw [->,line width=0.8pt] (2.312409987036266,0.) -- (3.672809219099011,-2.023370770064356);
	\draw [line width=0.8pt] (2.3118015931053515,-1.0194875995690844)-- (3.687590012963734,2.);
	\draw [->,line width=0.8pt] (2.3118015931053515,-1.0194875995690844) -- (3.687590012963734,-1.);
	\draw [line width=2.pt] (-4.580833035493351,-2.6108687372438015)-- (-0.9977224069976642,-2.6004223505718023);
	\draw [line width=2.pt] (0.976751104527751,-2.591669597353602)-- (4.559861733023438,-2.581223210681603);
	\draw [line width=2.pt] (-0.49585612643783666,-2.616490163162033)-- (0.5028204423655828,-2.616490163162033);
	\draw [line width=0.8pt] (-3.687590012963734,2.)-- (-2.3272978670955706,0.9781801421936286);
	\draw [line width=0.8pt] (-3.6875900129637342,0.)-- (-2.3272978670955706,0.9781801421936286);
	\draw [line width=0.8pt] (-3.687590012963734,-1.)-- (-2.3272978670955706,0.9781801421936286);
	\draw [line width=0.8pt] (-3.672614412416798,-2.02046159922395)-- (-2.3272978670955706,0.9781801421936286);
	\draw [line width=0.8pt] (-3.687590012963734,2.)-- (-2.312409987036266,0.);
	\draw [line width=0.8pt] (-3.671975610662866,1.)-- (-2.312409987036266,0.);
	\draw [line width=0.8pt] (-3.687590012963734,-1.)-- (-2.312409987036266,0.);
	\draw [line width=0.8pt] (-3.672614412416798,-2.02046159922395)-- (-2.312409987036266,0.);
	\draw [line width=0.8pt] (-3.687590012963734,2.)-- (-2.311616059483331,-1.022258289963095);
	\draw [line width=0.8pt] (-3.671975610662866,1.)-- (-2.311616059483331,-1.022258289963095);
	\draw [line width=0.8pt] (-3.672614412416798,-2.02046159922395)-- (-2.311616059483331,-1.022258289963095);
	\draw [line width=0.8pt] (-1.672480652362455,0.981804480686803)-- (-0.3124099870362662,0.);
	\draw [line width=0.8pt] (-1.688129116017763,-1.018345346116602)-- (-0.3124099870362662,0.);
	\draw [line width=0.8pt] (2.312409987036266,0.)-- (3.67270213290443,0.9781801421936286);
	\draw [line width=0.8pt] (2.3118015931053515,-1.0194875995690844)-- (3.67270213290443,0.9781801421936286);
	\draw [line width=0.8pt] (2.3257776205028176,0.9616732211173156)-- (3.6875900129637342,0.);
	\draw [line width=0.8pt] (2.3118015931053515,-1.0194875995690844)-- (3.6875900129637342,0.);
	\draw [line width=0.8pt] (2.3257776205028176,0.9616732211173156)-- (3.687590012963734,-1.);
	\draw [line width=0.8pt] (2.312409987036266,0.)-- (3.687590012963734,-1.);
	\draw [line width=0.8pt] (2.3257776205028176,0.9616732211173156)-- (3.672809219099011,-2.023370770064356);
	\draw [line width=0.8pt] (2.3118015931053515,-1.0194875995690844)-- (3.672809219099011,-2.023370770064356);
	\draw [line width=0.8pt] (2.3257776205028176,0.9616732211173156)-- (3.687590012963734,2.);
	\draw [->,line width=0.8pt] (2.319832405866583,-0.011039630830771835) -- (3.6847041472632425,1.993666296669693);
	\begin{scriptsize}
	\draw[color=black] (-2.7,-2.8) node {$Encoder$};
	\draw[color=black] (2.8,-2.8) node {$Decoder$};
	\draw[color=black] (0.0,-2.8) node {$Bottleneck$};
	\end{scriptsize}
	\end{tikzpicture}
\end{center}
\caption{The structure of a deep undercomplete autoencoder}
\label{fig:structure_of_ae}
\end{figure}

==> AEGR Article/Figures/Latent_variables.tex <==
\begin{figure*}
\begin{subfigure}{.20\textwidth}
  \centering
  % include first image
  \includegraphics[width=1.2\linewidth]{Figures/Full_InternetAds_AE_TrainingSet}  
  \caption{AE}
  \label{fig:lv-first}
\end{subfigure}
\hfil
\begin{subfigure}{.20\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.2\linewidth]{Figures/Full_InternetAds_AEGR_TrainingSet}  
  \caption{AEGR}
  \label{fig:lv-second}
\end{subfigure}
\hfil
\begin{subfigure}{.20\textwidth}
  \centering
  % include first image
  \includegraphics[width=1.2\linewidth]{Figures/Pruned_InternetAds_AE_TrainingSet}  
  \caption{AE (Pruned)}
  \label{fig:lv-third}
\end{subfigure}
\hfil
\begin{subfigure}{.20\textwidth}
  \centering
  % include second image
  \includegraphics[width=1.2\linewidth]{Figures/Pruned_InternetAds_AEGR_TrainingSet}  
  \caption{AEGR (Pruned)}
  \label{fig:lv-fourth}
\end{subfigure}
\caption{Visualisation plot of the latent variables (the first two features) extracted by a simple AE and also AEGR on InternetAds. The orange points represent anomalies while the blue points represent the normal points. The curves at the top and right side of each figure indicates the KDE curves.}
\label{fig:latent_variables}
\end{figure*}

==> AEGR Article/Figures/Simple_Structure.tex <==
\begin{figure}[!h]
	\begin{center}
		\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
		\clip(-3,-0.6) rectangle (3,.6);
		\draw [line width=0.8pt] (-2.,0.) circle (0.5);
		\draw [line width=0.8pt] (0.,0.) circle (0.5);
		\draw [line width=0.8pt] (2.,0.) circle (0.5);
		\draw [->,line width=1.pt] (-1.5,0.) -- (-0.5,0.);
		\draw [->,line width=1.pt] (0.5,0.) -- (1.5,0.);
		\begin{scriptsize}
		\draw[color=black] (-2,0) node {$x$};
		\draw[color=black] (0,0) node {$z$};
		\draw[color=black] (2,0) node {$y$};
		
		\draw[color=black] (-1.2,0.2) node {$u$};
		\draw[color=black] (0.85,0.2) node {$v$};
		\end{scriptsize}
		\end{tikzpicture}
	\end{center}
	\caption{The structure of a basic autoencoder}
	\label{fig:basic_ae}
\end{figure}

==> AEGR Article/Tables/AEGR_architecture.tex <==
\begin{table}
	\caption{The size of the middle layer for each dataset}
	\label{tab:aegr_architecture}
		\footnotesize
		\begin{tabularx}{\linewidth}{l l}
			\hline
			Dataset's name& \begin{tabular}[c]{@{}l@{}}Number of nodes in\\ the bottleneck\end{tabular}\\
			\hline
			PenDigits & 5 \\
			Shuttle & 4 \\
			Spambase & 8 \\
			InternetAds & 40 \\
			Arrhythmia & 17 \\
			NSLKDD & 12 \\
			UNSW-NB15 & 15 \\
			CTU13 & 7 \\
			\hline
		\end{tabularx}
\end{table}

==> AEGR Article/Tables/Datasets_details.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}
\caption{Details of the 8 datasets used in the experiments}
\label{tab:datasets_details}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c}
Data set name & \begin{tabular}[c]{@{}c@{}}No. of \\ features\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training \\ set\end{tabular} & \begin{tabular}[c]{@{}c@{}}Validation \\ set\end{tabular} & \begin{tabular}[c]{@{}c@{}}Testing \\ set\end{tabular} \\ \hline
PenDigits & 16 & 1247 & 312 & 727 \\
Shuttle & 9 & 3267 & 817 & 14500 \\
Arrhythmia & 259 & 251 & 83 & 86 \\
\hline
Spambase & 57 & 2759 & 919 & 923 \\
InternetAds & 1558 & 1414 & 471 & 474 \\
NSL-KDD(Probe) & 122 & 6319 & 1580 & 12132 \\
NSL-KDD(DoS) & 122 & 9060 & 2266 & 17169 \\
NSL-KDD(R2L) & 122 & 6183 & 1546 & 12598 \\
NSL-KDD(U2R) & 122 & 5428 & 1358 & 9778 \\
UNSW-NB15(Fuzzers) & 196 & 5934 & 1484 & 74184 \\
UNSW-NB15(Analysis) & 196 & 4640 & 1160 & 58000 \\
UNSW-NB15(Backdoor) & 196 & 4619 & 1155 & 57746 \\
UNSW-NB15(DoS) & 196 & 5460 & 1366 & 68264 \\
UNSW-NB15(Exploits) & 196 & 7151 & 1788 & 89393 \\
UNSW-NB15(Generic) & 196 & 7680 & 1920 & 96000 \\
UNSW-NB15(Reconnaissance) & 196 & 5319 & 1330 & 66491 \\
UNSW-NB15(Shellcode) & 196 & 4570 & 1143 & 57133 \\
UNSW-NB15(Worm) & 196 & 4584 & 1146 & 56130 \\
CTU13-13(Virut) & 40 & 4315 & 1438 & 1440 \\
CTU13-10(Rbot) & 38 & 7331 & 2443 & 2445 \\
CTU13-09(Neris) & 41 & 12895 & 4298 & 4301 \\
CTU13-08(Murlo) & 40 & 8045 & 2681 & 2683 \\
\hline
\end{tabular}%
}
\end{table}

==> AEGR Article/Tables/NSLKDD.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \cellcolor[HTML]{C0C0C0}
\begin{table*}
\centering
\caption{PR AUC and ROC AUC for NSL-KDD and CTU13}
\label{tab:NSLKDD}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Detection approach} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Modification\\ method\end{tabular}} & \multicolumn{2}{c|}{DoS} & \multicolumn{2}{c|}{Probe} & \multicolumn{2}{c|}{R2L} & \multicolumn{2}{c|}{U2R} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Virut\\ CTU13-13\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Rbot\\ CTU13-10\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Neris\\ CTU13-09\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Murlo\\ CTU13-08\end{tabular}} \\ \cline{3-18} 
 &  & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} \\ \hline
Stand-alone LOF & None & 0.549 & 0.555 & 0.830 & 0.635 & 0.810 & 0.687 & 0.994 & 0.530 & 0.644 & 0.781 & 0.845 & 0.465 & 0.708 & 0.060 & 0.940 & 0.594 \\ \hline

AE-RE & None & 0.547 & 0.440 & 0.800 & 0.056 & 0.790 & 0.543 & 0.994 & 0.569 & 0.431 & 0.463 & 0.815 & 0.057 & 0.864 & 0.003 & 0.920 & 0.001 \\ \hline

\multirow{3}{*}{AE-LOF} & None & 0.522 & 0.492 & 0.821 & 0.645 & 0.756 & 0.525 & 0.994 & 0.551 & 0.439 & 0.558 & 0.807 & 0.254 & 0.747 & 0.199 & 0.933 & 0.564 \\ \cline{2-18} 

 & Pruning & 0.549 & 0.512 & 0.895 & 0.742 & 0.757 & 0.409 & 0.994 & 0.516 & 0.371 & 0.412 & 0.799 & 0.241 & 0.981 & 0.880 & \cellcolor[HTML]{C0C0C0}0.988 & \cellcolor[HTML]{C0C0C0}0.908 \\ \cline{2-18} 
 
 & Pruning+DA & 0.687 & 0.781 & 0.683 & 0.296 & 0.766 & 0.548 & 0.993 & 0.451 & 0.518 & 0.639 & 0.895 & 0.523 & 0.966 & 0.900 & 0.800 & 0.068 \\ \hline
 
\multirow{3}{*}{AEGR-LOF} & None & 0.514 & 0.488 & 0.844 & 0.677 & 0.823 & 0.679 & 0.997 & 0.789 & 0.552 & 0.699 & 0.857 & 0.514 & 0.719 & 0.088 & 0.928 & 0.577 \\ \cline{2-18} 

 & Pruning & \cellcolor[HTML]{C0C0C0}0.925 & \cellcolor[HTML]{C0C0C0}0.883 & \cellcolor[HTML]{C0C0C0}0.947 & \cellcolor[HTML]{C0C0C0}0.841 & \cellcolor[HTML]{C0C0C0}0.859 & \cellcolor[HTML]{C0C0C0}0.685 & \cellcolor[HTML]{C0C0C0}0.998 & \cellcolor[HTML]{C0C0C0}0.817 & 0.472 & 0.588 & \cellcolor[HTML]{C0C0C0}0.899 & 0.547 & 0.891 & 0.452 & 0.979 & 0.782 \\ \cline{2-18} 
 
 & Pruning+DA & 0.643 & 0.695 & 0.797 & 0.598 & 0.674 & 0.287 & 0.993 & 0.550 & \cellcolor[HTML]{C0C0C0}0.797 & \cellcolor[HTML]{C0C0C0}0.832 & 0.859 & \cellcolor[HTML]{C0C0C0}0.597 & \cellcolor[HTML]{C0C0C0}0.992 & \cellcolor[HTML]{C0C0C0}0.985 & 0.917 & 0.332 \\ \hline
\end{tabular}%
}
\end{table*}

==> AEGR Article/Tables/Single-type.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \cellcolor[HTML]{C0C0C0}

\begin{table*}
\centering
\caption{PR AUC and ROC AUC for data sets with single-type anomaly}
\label{tab:single-type}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Detection approach} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Modification\\ method\end{tabular}} & \multicolumn{2}{c|}{Spambase} & \multicolumn{2}{c|}{InternetAds} & \multicolumn{2}{c|}{PenDigits} & \multicolumn{2}{c|}{Shuttle} & \multicolumn{2}{c|}{Arrhythmia} \\ \cline{3-12} 
 &  & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} \\ \hline
 
Stand-alone LOF & None & 0.596 & 0.418 & 0.857 & 0.498 & 0.554 & 0.529 & 0.700 & 0.343 & 0.638 & 0.626 \\ \hline

AE-RE & None & 0.606 & 0.324 & 0.838 & 0.188 & 0.483 & 0.368 & 0.792 & 0.007 & 0.558 & 0.289 \\ \hline

\multirow{3}{*}{AE-LOF} & None & 0.579 & 0.428 & 0.853 & 0.515 & 0.574 & 0.590 & 0.819 & 0.689 & 0.681 & 0.678\\ \cline{2-12} 

 & Pruning & 0.650 & 0.497 & 0.909 & 0.638 & 0.980 & 0.970 & \cellcolor[HTML]{C0C0C0}0.839 & \cellcolor[HTML]{C0C0C0}0.720 & 0.703 & 0.688 \\ \cline{2-12} 
 
 & Pruning+DA & 0.503 & 0.334 & 0.859 & 0.538 & 0.315 & 0.078 & 0.635 & 0.105 & 0.605 & 0.616 \\ \hline
 
\multirow{3}{*}{AEGR-LOF} & None & 0.551 & 0.377 & 0.854 & 0.521 & 0.491 & 0.499 & 0.689 & 0.398 & 0.698 & 0.671 \\ \cline{2-12} 

 & Pruning & 0.558 & 0.388 & \cellcolor[HTML]{C0C0C0}0.928 & \cellcolor[HTML]{C0C0C0}0.687 & \cellcolor[HTML]{C0C0C0}0.998 & \cellcolor[HTML]{C0C0C0}0.998 & 0.696 & 0.414 & \cellcolor[HTML]{C0C0C0}0.728 & \cellcolor[HTML]{C0C0C0}0.732 \\ \cline{2-12} 
 
 & Pruning+DA & \cellcolor[HTML]{C0C0C0}0.682 & \cellcolor[HTML]{C0C0C0}0.646 & 0.854 & 0.538 & 0.970 & 0.958 & 0.812 & 0.559 & 0.512 & 0.484 \\ \hline
\end{tabular}%
}
\end{table*}

==> AEGR Article/Tables/UNSW.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \cellcolor[HTML]{C0C0C0}
\begin{table*}
\centering
\caption{The PR AUC and ROC AUC values for UNSW-NB15}
\label{tab:UNSW}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Detection approach} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Modification\\ method\end{tabular}} & \multicolumn{2}{c|}{Fuzzers} & \multicolumn{2}{c|}{Analysis} & \multicolumn{2}{c|}{DoS} & \multicolumn{2}{c|}{Exploits} & \multicolumn{2}{c|}{Generic} & \multicolumn{2}{c|}{Reconnaissance} & \multicolumn{2}{c|}{Shellcode} & \multicolumn{2}{c|}{Worms} \\ \cline{3-18} 

 &  & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} & \multicolumn{1}{c|}{PR} & \multicolumn{1}{c|}{ROC} \\ \hline
 
Stand-alone LOF & None & 0.793 & 0.562 & 0.983 & 0.702 & \cellcolor[HTML]{C0C0C0}0.926 & \cellcolor[HTML]{C0C0C0}0.778 & 0.667 & 0.603 & 0.583 & 0.499 & 0.872 & 0.590 & 0.986 & 0.618 & \cellcolor[HTML]{C0C0C0}1.000 & 0.846 \\ \hline

AE-RE & None & 0.722 & 0.329 & 0.97 & 0.593 & 0.853 & 0.584 & 0.605 & 0.443 & 0.687 & 0.624 & 0.873 & 0.572 & 0.981 & 0.589 & 0.998 & 0.091 \\ \hline

\multirow{3}{*}{AE-LOF} & None & 0.786 & 0.520 & 0.986 & 0.720 & 0.862 & 0.589 & 0.633 & 0.506 & 0.563 & 0.463 & 0.869 & 0.557 & 0.987 & 0.627 & \cellcolor[HTML]{C0C0C0}1.000 & 0.877 \\ \cline{2-18} 
 & Pruning & 0.791 & 0.568 & 0.983 & 0.721 & 0.863 & 0.569 & 0.654 & 0.537 & 0.574 & 0.518 & 0.850 & 0.475 & 0.980 & 0.517 & \cellcolor[HTML]{C0C0C0}1.000 & 0.881 \\ \cline{2-18} 
 & Pruning+DA & 0.646 & 0.205 & 0.940 & 0.381 & 0.815 & 0.422 & 0.569 & 0.374 & 0.377 & 0.012 & 0.858 & 0.538 & \cellcolor[HTML]{C0C0C0}0.996 & \cellcolor[HTML]{C0C0C0}0.850 & \cellcolor[HTML]{C0C0C0}1.000 & 0.750 \\ \hline
 
\multirow{3}{*}{AEGR-LOF} & None & 0.785 & 0.532 & \cellcolor[HTML]{C0C0C0}0.998 & 0.948 & 0.858 & 0.601 & 0.620 & 0.499 & 0.597 & 0.518 & 0.858 & 0.538 & 0.988 & 0.632 & \cellcolor[HTML]{C0C0C0}1.000 & 0.861 \\ \cline{2-18} 
 & Pruning & 0.810 & 0.574 & \cellcolor[HTML]{C0C0C0}0.998 & \cellcolor[HTML]{C0C0C0}0.955 & 0.848 & 0.543 & 0.601 & 0.475 & 0.674 & 0.626 & 0.841 & 0.467 & 0.979 & 0.485 & \cellcolor[HTML]{C0C0C0}1.000 & \cellcolor[HTML]{C0C0C0}0.902 \\ \cline{2-18} 
 & Pruning+DA & \cellcolor[HTML]{C0C0C0}0.833 & \cellcolor[HTML]{C0C0C0}0.576 & 0.986 & 0.698 & 0.876 & 0.697 & \cellcolor[HTML]{C0C0C0}0.742 & \cellcolor[HTML]{C0C0C0}0.655 & \cellcolor[HTML]{C0C0C0}0.879 & \cellcolor[HTML]{C0C0C0}0.758 & \cellcolor[HTML]{C0C0C0}0.945 & \cellcolor[HTML]{C0C0C0}0.772 & 0.991 & 0.726 & 0.999 & 0.342\\ \hline
 
\end{tabular}%
}
\end{table*}
